FedTDP: A Privacy-Preserving and Unified Framework for Trajectory Data Preparation via Federated Learning

Trajectory data, which capture the movement patterns of people and vehicles over time and space, are crucial for applications like traffic optimization and urban planning. However, issues such as noise and incompleteness often compromise data quality, leading to inaccurate trajectory analyses and limiting the potential of these applications. While Trajectory Data Preparation (TDP) can enhance data quality, existing methods suffer from two key limitations: (i) they do not address data privacy concerns, particularly in federated settings where trajectory data sharing is prohibited, and (ii) they typically design task-specific models that lack generalizability across diverse TDP scenarios. To overcome these challenges, we propose FedTDP, a privacy-preserving and unified framework that leverages the capabilities of Large Language Models (LLMs) for TDP in federated environments. Specifically, we: (i) design a trajectory privacy autoencoder to secure data transmission and protect privacy, (ii) introduce a trajectory knowledge enhancer to improve model learning of TDP-related knowledge, enabling the development of TDP-oriented LLMs, and (iii) propose federated parallel optimization to enhance training efficiency by reducing data transmission and enabling parallel model training. Experiments on 6 real datasets and 10 mainstream TDP tasks demonstrate that FedTDP consistently outperforms 13 state-of-the-art baselines.

==> 2_related.tex <==
\vspace{-4mm}
\section{Related Work}
\vspace{-2mm}
\label{sec:related}

\textbf{Trajectory Data Preparation.}
Numerous TDP methods have been proposed to improve trajectory data quality. For the anomalous detection task, ATROM~\cite{qg23} introduces a new probabilistic metric learning model to enable anomaly recognition in complex environments. 
For the trajectory imputation task, Kamel~\cite{mm23} proposes a scalable system that inserts additional real trajectory points to enhance model accuracy. 
For the map matching task, GraphMM~\cite{yl24} effectively utilizes both road network and trajectory features to improve map matching accuracy. 
For the trajectory-user link task, AttnTUL~\cite{wc24} introduces a novel hierarchical spatio-temporal attention neural network to establish links between trajectories and users accurately. 
For the travel mode identification task, Estimator~\cite{hdl24} partitions the traffic space into disjoint spatial regions to enhance the precision of travel mode identification. 
For the trajectory simplification task, S3~\cite{zqf23} proposes a lightweight framework with two chained Seq2Seq modules to enable self-supervised trajectory simplification. 
For the trajectory recovery task, LightTR~\cite{zql24} presents a local trajectory embedding module, to offer higher computational efficiency while maintaining feature extraction capabilities.
However, none of these studies have considered data privacy constraints. They typically assume that the trajectory data collection is centralized, which introduces a significant risk of privacy leakage, especially in federated environments. In addition, all of them are single-task methods. When handling multiple TDP tasks, different models need to be trained for each specific task. It not only demands substantial time and computational resources but also results in poor model generalization ability. \textbf{\textit{In contrast, we aim to propose a privacy-preserving and unified framework to support various trajectory data preparation tasks while safeguarding trajectory data privacy.}}

% \begin{table}[tb]
%     \centering
%     \vspace{-2mm}
%     \caption{Notation and Description}
%     \resizebox{\linewidth}{!}{\begin{tabular}{cl}
%     \hline
%          \textbf{Notation} & \textbf{Description} \\ \hline
%          $p$ & A spatio-temporal point $\langle l,t \rangle$ \\ 
%          $T$ & A trajectory with multiple points $\{p_1,p_2,\ldots\}$ \\ 
%          $\textit{ST}$ & A sub-trajectory of a trajectory $T$\\  
%          $u$ & A user that represents a trajectory $T$\\ 
%          $U$ & A set of users $\{u_1, u_2,\ldots\}$ \\ 
%          $S$ & A data silo that represents a region\\ 
%          $C$ & A client that represents a region\\ 
%          $D$ & The trajectory database in a client $C$\\ 
%          $F$ & The horizontal federation with data silos $\{S_1, S_2,\ldots\}$ \\ 
%          $\theta_\textit{LLM}$,$\theta_\textit{SLM}$ & The large language model and small language model\\
%          $\mathcal{C}$ & A set of clients $\{C_1, C_2,\ldots\}$ \\ 
%          $\mathcal{D}$ & The collection of spatio-temporal points $\{D_1, D_2, \ldots\}$\\
%          \hline
%     \end{tabular}}
%     \label{tab:notation}
%     \vspace{-8mm}
% \end{table}

\vspace{-1mm}
\textbf{LLMs for Other Data Preparation.}
A few works on table data preparation using LLMs have been proposed recently. For instance, MELD~\cite{myy24} leverages a mixture-of-experts architecture to support merging and augmentation of domain-specific experts trained on limited annotated examples. Similarly, TableGPT~\cite{pl24} presents a table-tuning paradigm to enhance the model's ability on understanding and processing table-related tasks. Additionally,~\cite{an22} explores and evaluates the performance of LLMs on five table data cleaning and integration tasks through prompt-based methods.
However, these works are specifically tailored for table DP and are not directly applicable to TDP tasks. They lack the necessary understanding of trajectory data and do not account for the spatio-temporal characteristics and complexity of TDP tasks, making them unsuitable for such applications. \textbf{\textit{In contrast, we aim to develop a TDP-oriented LLM to effectively support various trajectory data preparation tasks.}}


